REQUAL-LM: Reliability and Equity through Aggregation in Large Language Models

The extensive scope of large language models (LLMs) across various domains underscores the critical importance of responsibility in their application, beyond natural language processing. In particular, the randomized nature of LLMs, coupled with inherent biases and historical stereotypes in data, raises critical concerns regarding reliability and equity. Addressing these challenges are necessary before using LLMs for applications with societal impact. Towards addressing this gap, we introduce REQUAL-LM, a novel method for finding reliable and equitable LLM outputs through aggregation. Specifically, we develop a Monte Carlo method based on repeated sampling to find a reliable output close to the mean of the underlying distribution of possible outputs. We formally define the terms such as reliability and bias, and design an equity-aware aggregation to minimize harmful bias while finding a highly reliable output. REQUAL-LM does not require specialized hardware, does not impose a significant computing load, and uses LLMs as a blackbox. This design choice enables seamless scalability alongside the rapid advancement of LLM technologies. Our system does not require retraining the LLMs, which makes it deployment ready and easy to adapt. Our comprehensive experiments using various tasks and datasets demonstrate that REQUAL- LM effectively mitigates bias and selects a more equitable response, specifically the outputs that properly represents minority groups.

==> details.tex <==
\section{Technical Details}

\subsection{Gender Bias Scoring}\label{sec:demoEmbed}


Sentences can be represented to encapsulate the semantic of human language. Nevertheless, acquiring a vector specifically representing gender as an abstract concept is challenging. Instead certain terms are inherently linked with a gender. To quantify gender at the sentence level, one approach involves employing simple sentences that exclusively feature gender associated words. \cite{seat} utilizes simple sentences constructed from words and terms provided by \cite{weat}. These sentences do not contain any contextual information beyond fundamental gender-related terms, such as "She is here," "He is here," "He is a man," "She is a woman," and so forth. Their finding demonstrate that the embedded vectors encapsulate the encoded gender bias inherent in respective sentences. 
We define the vector $\vec{x}_i = (x_1, x_2, x_3, ..., x_n)$ as a representation for sentence $i$, derived from the InstructorOR model \cite{Instructor}. The InstructorOR model is a multi-task model designed to generate task-specific embeddings in accordance with provided instructions. Given a set $X$ of sentences associated with a particular gender, we compute the gender attribute vector as
\begin{equation}
  k \in \{\textit{female}, \textit{male}\}:~  \vec{v}_{k} = \textit{mean}_{x_i \in X}(\vec{x_i}) 
\end{equation}



% Given a set of black box large language model, obtaining query is straight forward. However, the task of selecting a proper output for a user specified purpose is challenging. In this work we aim to define the problem of selecting an output from the perspective of fairness. 
% In the context of this study, our primary objective is to quantify gender bias within geometric space through the utilization of sentence embeddings that encapsulate textual content and associated gender-related attributes. The process of acquiring sentence embeddings is a relatively straightforward task through the use of an encoder. Nevertheless, it is essential to recognize that gender is an abstract concept, and the most basic approach involves leveraging pre-trained word embeddings designed to encode gender information. However, our specific requirement entails the generation of sentence embeddings that facilitate the measurement of proximity to the target sentence embedding. 
% Motivated by \citep{adept}, we have assembled a corpus of straightforward sentences devoid of any contextual information beyond fundamental gender-related terms, such as "She is here," "He is here," "He is a man," "She is a woman," and so forth. 

% These sentences serve as the source for generating embeddings. By computing the average embedding within the collection of sentences linked to each gender category, we can derive distinct embeddings for each gender attribute.

% Foremost, for the acquisition of gender sentence embeddings, we employ the InstructOR Model \citep{Instructor}. 

% This procedure is a one-time operation, wherein the resultant attribute vectors may be persistently archived for future applications. 
The gender orientation of a sentence is gauged through the cosine similarity between the vectors representing the sentence and its attribute embedding. Past studies have demonstrated that cosine similarity effectively encapsulates the semantic relevance between textualized contents \cite{seat, weat, stereoset}. Nonetheless, it is imperative to acknowledge that cosine similarity is not without its limitations. Nonetheless, as demonstrated by the study conducted by \citep{biasWordRep}, it is evident that the conventional employment of cosine similarity is inadequate for the accurate computation of bias. Notably, we characterize bias as the extent to which a sentence portrays a minority group, and the disparity between two cosine similarity scores is considered indicative of this bias. Consequently, we introduce a \textit{Gender Bias Scoring (GBS)}, $b_i$, for query $i$ as follows:
\begin{gather}\label{weighting}
    b_i = \cos(\vec{v}_{majority}, \vec{v}_i) - \cos(\vec{v}_{minority}, \vec{v}_i)\\
    w_i = 1 - b_i
\end{gather}
    
The bias score is employed to determine the weight, denoted as $w_i$, assigned to each query. This weight, $w_i$, reflects that as a vector embedding tends more towards the majority group, the associated bias score $b_i$ diminishes. In Example ~\ref{ex-1}, where the objective is to enhance diversity and mitigate disparity, it is necessary to allocate a greater weight to sets featuring a higher number of female employees. However, this weighting metric requires an adjustment to the bias score sign based on the specified task. In instances where the query exhibits a stereotype towards the minority group, it is evident that a lower weight should be assigned to queries characterized by a lower bias score  (~$\cos(\vec{v}_{majority}, \vec{v}_i) <  \cos(\vec{v}_{minority}, \vec{v}_i)$~). Thus, the weighting will be modified as $w_i = b_i -1$.
% \section{Racial Bias Scoring}

% Racial terms are non-binary and this makes it hard to obtain a final bias score. For a set of racial term, compute cosine similarity for each output. Take the maximum for each output. Compute the similarity of the output with pleasant and unpleasant embedding and take the difference. The bias score will be the multiplication of bias and the last term computed. 



\subsection{Query Selection}

In this section, we articulate the incorporation of Gender Bias Score (GBS) within a multi-model framework to produce outputs characterized by fairness, gender neutrality, and/or diversity according to the specified task. A pivotal aspect of our framework lies in its ability to leverage language models as black boxes. This entails the utilization of powerful closed-source language models across a diverse spectrum, enabling the selection of the most appropriate output. We simulate a pseudo-ensemble model that queries multiple models, generating diverse outputs by adjusting parameters that govern the model's creativity and novelty. The parameters considered in our experiments include temperature, frequency penalty, and presence penalty. Each output is assigned a weight using GBS, as outlined in Equation \ref{weighting}, signifying the importance of each individual output in the final response selection process. 


% By employing a singular model and modulating two essential parameters, namely temperature and repetition penalty, we elicit diverse outcomes. Subsequently, to assess the responses in the context of their sensitive attributes, we leverage the cosine similarity metric, capitalizing on the inherent property that semantically akin sentences display proximal vectors within the vector space, thereby yielding higher cosine similarity scores. 
Given a set of output embeddings from N models each weighted by their respective bias scores, denoted as $\{w_1 \cdot \vec{v}_1, w_2 \cdot \vec{v}_2, ..., w_N \cdot \vec{v}_N\}$, the centroid of the output cluster, denoted as $\vec{v}_c$, is computed as the weighted average of these vectors.

\begin{equation}
    \Vec{v}_c = \frac{1}{N}\sum_{i =1}^{N} w_i *\vec{v}_i
\end{equation}
% In certain instances where gender-specific terms are utilized without any accompanying stereotype or contextual bias, the resulting sentence embeddings inherently exhibit higher cosine similarity concerning either male or female embedding. To mitigate this concern, a proposed approach entails assessing the disparity between the cosine similarities associated with male and female embeddings. This differential measure serves as an indicator of the extent to which a sentence inclines toward a particular gender, with an optimal value of 0 in cases where $ Cosin_{female} = Cosin_{male}$

% In this study, we explore the correspondence between the output embedding derived from the InstructOR Model and the gender-related attributes, specifically focusing on the gender orientation expressed within the output. This metric reflects the degree to which our outputs exhibit gender bias and employ gender-associated vocabulary. To quantify this bias, we normalize the score by substituting the minimum cosine similarity value among all the outputs and dividing it by the range of similarity scores, denoted as the score interval length:
% \begin{equation}
%     Score_{i} = \frac{Cosine(Output_{i} - \min Cosine) }{ \max Cosine - \min Cosine} 
% \end{equation}

The weighted centroid $\Vec{v}$ is influenced by the weights assigned to each output vector. Output vectors with smaller weights contribute less to the centroid, reflecting their reduced impact on the overall representation. Consequently, the output vector in the embedding space that is closest to this centroid is indicative of a more fair response, as it is less influenced by outputs with smaller weights, which correspond to lower bias measures. In contrast, an output closer to the unweighted centroid $\Vec{v}^{'} = \frac{1}{N}\sum_{i =1}^{N} \vec{v}_i$ may be more influenced by outputs with higher bias measures, potentially resulting in a less fair representation. 

% To aggregate the outputs and derive a single output vector that encapsulates both the most and moderately biased sentences, we compute the average across the output embeddings. In this process, each $Output_{i}$ is weighted by multiplying it by its corresponding coefficient, calculated as $1 - Score_{i}$.


\subsection{Observations}
% Without the repetition penalty, the outputs using API will not be different in many cases.
% If that happens, the majority response will be the final output regardless of the bias score.


